Pixel Recursive Super Resolution

We present a pixel recursive super resolution model that synthesizes realistic details into images while enhancing their resolution. A low resolution image may correspond to multiple plausible high resolution images, thus modeling the super resolution process with a pixel independent conditional model often results in averaging different details--hence blurry edges. By contrast, our model is able to represent a multimodal conditional distribution by properly modeling the statistical dependencies among the high resolution image pixels, conditioned on a low resolution input. We employ a PixelCNN architecture to define a strong prior over natural images and jointly optimize this prior with a deep conditioning convolutional network. Human evaluations indicate that samples from our proposed model look more photo realistic than a strong L2 regression baseline.

==> rebuttal/rebuttal_table.tex <==
% Created with //google3/experimental/users/rld/calculate_algo_metrics.py
\begin{center}
\begin{tabular}{r|ccccc}
Algorithm  &  MS-SSIM & Consistency & \% Fooled\\
\hline
\hline 
 Bicubic    & 0.76             &  0.006   & -- \\
 NN         & 0.66             &  0.024      & -- \\
 Regression &  \bf 0.90 &  \bf 0.004         & $4.0\pm0.2$  \\
 $\tau=1.0$ &  0.86             &  0.008        & $\bf 11.0\pm0.1$ \\
 \hline 
 Bicubic    &  0.70      & \bf  0.002    & -- \\
 NN         &  0.45          & 0.040    & -- \\
 Regression &  \bf 0.75  & 0.003     & $2.1\pm0.1$      \\
 $\tau=1.2$ &  0.58          & 0.018   & $\bf 27.9\pm0.3$     \\[-.4cm]
\end{tabular}
\end{center}
% faces bicubic
% MSE truth 0.000
% MSE bicubic 0.006
% MSE nearest_neighbors_L2 0.024
% MSE baselineL2 0.004
% MSE mask100 0.008
% MSE mask110 0.008
% MSE mask120 0.008
% 
% bedrooms bicubic
% MSE truth 0.014
% MSE bicubic 0.002
% MSE nearest_neighbors_L2 0.040
% MSE baselineL2 0.003
% MSE mask100 0.016
% MSE mask110 0.017
% MSE mask120 0.018

\caption{Top: CelebA dataset. Bottom: LSUN bedrooms dataset. Consistency is the MSE between the input low-res image and a downsampled sample. NN refers to the nearest neighbor baseline.}
\label{tab:results}


==> toy.tex <==
\begin{figure}
Dataset
\begin{center}
\includegraphics[width=.45\textwidth]{Data-Model.pdf}
\end{center}


{
  \small
\begin{tabular}{c@{\hspace{.1cm}}rc@{\hspace{.1cm}}c@{\hspace{.1cm}}c@{\hspace{.1cm}}c@{\hspace{.1cm}}}

% \multicolumn{5}{l}{\bf Dataset}\\
% \bf Dataset & & & & \\
 \hline \\

 & \raisebox{.5cm}{Input}  & {\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_0_1.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_1_1.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_2_1.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_3_1.png}} \\ 
\parbox[t]{6mm}{\multirow{3}{*}{\rotatebox{90}{Model Output}}} &
 \raisebox{.5cm}{Cross-entropy}  & {\includegraphics[width=.14\linewidth]{multimodal_numpy/xentropy_0_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/xentropy_1_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/xentropy_2_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/xentropy_3_0.png}} \\ 
& \raisebox{.5cm}{$L_2$ Regression}  & {\includegraphics[width=.14\linewidth]{multimodal_numpy/regression_0_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/regression_1_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/regression_2_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/regression_3_0.png}} \\ 
& \raisebox{.5cm}{PixelCNN}  & {\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_0_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_1_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_2_0.png}} &{\includegraphics[width=.14\linewidth]{multimodal_numpy/pixelcnn_3_0.png}} \\ 
\end{tabular}
}

\caption{Top: A cartoon of how the input and output pairs
  for the toy dataset were created.
  Bottom: Example predictions for various algorithms trained on this
  dataset. The pixel independent $L_2$ regression and
  cross-entropy models do not exhibit multimodal predictions. 
  The PixelCNN output is stochastic and multiple samples will place a digit in
  either corner 50\% of the time.}
\label{fig:toy}
\end{figure}

